Improving the quality of generative models through Smirnov transformation

Solving the convergence issues of Generative Adversarial Networks (GANs) is one of the most outstanding problems in generative models. In this work, we propose a novel activation function to be used as output of the generator agent. This activation function is based on the Smirnov probabilistic transformation and it is specifically designed to improve the quality of the generated data. In sharp contrast with previous works, our activation function provides a more general approach that deals not only with the replication of categorical variables but with any type of data distribution (continuous or discrete). Moreover, our activation function is derivable and therefore, it can be seamlessly integrated in the backpropagation computations during the GAN training processes. To validate this approach, we evaluate our proposal against two different data sets: a) an artificially rendered data set containing a mixture of discrete and continuous variables, and b) a real data set of flow-based network traffic data containing both normal connections and cryptomining attacks. To evaluate the fidelity of the generated data, we analyze both their results in terms of quality measures of statistical nature and also regarding the use of these synthetic data to feed a nested machine learning-based classifier. The experimental results evince a clear outperformance of the GAN network tuned with this new activation function with respect to both a na\"ive mean-based generator and a standard GAN. The quality of the data is so high that the generated data can fully substitute real data for training the nested classifier without a fall in the obtained accuracy. This result encourages the use of GANs to produce high-quality synthetic data that are applicable in scenarios in which data privacy must be guaranteed.

==> figuras/FIG_CR_baseline.tex <==
\begin{figure*}[!h]
\begin{mdframed}
\centering

\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/Mix_test_CR_B_R.png} 
  \includegraphics[width=0.49\linewidth]{images/Mix_tr_CR_B_R.png}}
\caption{Real data.}\label{fig:Mix_CR_B_R}
\end{subfigure}
%
\medskip

\begin{subfigure}[t]{.99\textwidth}
\centering
\vspace{0pt}% set the real top as the top
\includegraphics[width=0.49\linewidth]{images/Mix_test_CR_B_M.png}
\hfill
\includegraphics[width=0.49\linewidth]{images/Mix_tr_CR_B_M.png}
\caption{Naive generator with means.}\label{fig:Mix_CR_B_M}
\end{subfigure}

%
\end{mdframed}
\medskip
\begin{minipage}[t]{.99\textwidth}
\caption{$F_1$-score on testing (left) and training (right) using real data (DS1)    \ref{fig:Mix_CR_B_R}) and naive noise generator with means \ref{fig:Mix_CR_B_M}) on training. Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented. Experiment was run 100 times.} \label{fig:Mix_CR_B}
\end{minipage}

\end{figure*}

==> figuras/FIG_CR_et0.tex <==


\begin{figure*}[!t]

\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/Dist_CR_et0_FA_L.png} 
\caption{$L^1$ distance}
\label{fig:vainilla-f1}
\end{subfigure}
%
\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/Jacc_CR_et0_FA_L.png} 
\caption{Jaccard index}
\label{fig:vainilla-kolmo}
\end{subfigure}
%
%\medskip
%
\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/F1_tr_CR_et0_FA_L.png} 
\caption{$F_1$-score on DS1}
\label{fig:vainilla-jac}
\end{subfigure}
%
\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/F1_test_CR_et0_FA_L.png} 
\caption{$F_1$-score on DS2}
\label{fig:vainilla-jac-1}
\end{subfigure}

\medskip

\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/Dist_CR_et0_FA_S.png} 
\caption{$L^1$ distance}
\label{fig:vainilla-f1}
\end{subfigure}
%
\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/Jacc_CR_et0_FA_S.png} 
\caption{Jaccard index}
\label{fig:vainilla-kolmo}
\end{subfigure}
%
%\medskip
%
\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/F1_tr_CR_et0_FA_S.png} 
\caption{$F_1$-score on DS1}
\label{fig:vainilla-jac}
\end{subfigure}
%
\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/F1_test_CR_et0_FA_S.png} 
\caption{$F_1$-score on DS2}
\label{fig:vainilla-jac-1}
\end{subfigure}


\caption{Evolution of  $L^1$ distance, Jaccard index, $F_1$-score on training and testing, using GAN generator with linear activation (top row) and custom activation (bottom row) for label 0. The $x$-axis represents the GAN training epochs. hay que ponerlostodos los ejes Y a las mismas escalas}
\label{fig:CR_et0}
\end{figure*}


==> figuras/FIG_CR_et1.tex <==


\begin{figure*}[!t]

\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/Dist_CR_et1_FA_L.png} 
\caption{$L^1$ distance}
\label{fig:vainilla-f1}
\end{subfigure}
%
\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/Jacc_CR_et1_FA_L.png} 
\caption{Jaccard index}
\label{fig:vainilla-kolmo}
\end{subfigure}
%
%\medskip
%
\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/F1_tr_CR_et1_FA_L.png} 
\caption{$F_1$-score on DS1}
\label{fig:vainilla-jac}
\end{subfigure}
%
\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/F1_test_CR_et1_FA_L.png} 
\caption{$F_1$-score on DS2}
\label{fig:vainilla-jac-1}
\end{subfigure}

\medskip

\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/Dist_CR_et1_FA_S.png} 
\caption{$L^1$ distance}
\label{fig:vainilla-f1}
\end{subfigure}
%
\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/Jacc_CR_et1_FA_S.png} 
\caption{Jaccard index}
\label{fig:vainilla-kolmo}
\end{subfigure}
%
%\medskip
%
\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/F1_tr_CR_et1_FA_S.png} 
\caption{$F_1$-score on DS1}
\label{fig:vainilla-jac}
\end{subfigure}
%
\begin{subfigure}[t]{.245\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/F1_test_CR_et1_FA_S.png} 
\caption{$F_1$-score on DS2}
\label{fig:vainilla-jac-1}
\end{subfigure}


\caption{Evolution of  $L^1$ distance, Jaccard index, $F_1$-score on training and testing, using GAN generator with linear activation (top row) and custom activation (bottom row) for label 1. The $x$-axis represents the GAN training epochs. hay que ponerlostodos los ejes Y a las mismas escalas}
\label{fig:CR_et1}
\end{figure*}


==> figuras/__FIG_CR_et0_Distr.tex <==

%%%%%%%%%
% et0
%%%%%%%%%

\begin{figure*}[!t]
\centering
%et0
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F0_CR_et0_REAL.png} 
\caption{Feat 0. Real data.}\label{fig:CR-distr-real-l0-f0}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F0_CR_et0_FA_l.png} 
\caption{Feat 0. Linear activation.}\label{fig:CR-distr-LA-l0-f0}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F0_CR_et0_FA_S.png} 
\caption{Feat 0. Custom activation.}\label{fig:CR-distr-LS-l0-f0}
\end{subfigure}

\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F1_CR_et0_REAL.png} 
\caption{Feat 1. Real data.}\label{fig:CR-distr-real-l0-f1}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F1_CR_et0_FA_l.png} 
\caption{Feat 1. Linear activation.}\label{fig:CR-distr-LA-l0-f1}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F1_CR_et0_FA_S.png} 
\caption{Feat 1. Custom activation.}\label{fig:CR-distr-LS-l0-f1}
\end{subfigure}

\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F2_CR_et0_REAL.png} 
\caption{Feat 2. Real data.}\label{fig:CR-distr-real-l0-f2}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F2_CR_et0_FA_l.png} 
\caption{Feat 2. Linear activation.}\label{fig:CR-distr-LA-l0-f2}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F2_CR_et0_FA_S.png} 
\caption{Feat 2. Custom activation.}\label{fig:CR-distr-LS-l0-f2}
\end{subfigure}

\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F3_CR_et0_REAL.png} 
\caption{Feat 3. Real data.}\label{fig:CR-distr-real-l0-f3}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F3_CR_et0_FA_l.png} 
\caption{Feat 3. Linear activation.}\label{fig:CR-distr-LA-l0-f3}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F3_CR_et0_FA_S.png} 
\caption{Feat 3. Custom activation.}\label{fig:CR-distr-LS-l0-f3}
\end{subfigure}

\caption{Frequency distribution histogram of the 4 variables extracted from normal traffic (Label 0). Real data distribution: \ref{fig:CR-distr-real-l0-f0}, \ref{fig:CR-distr-real-l0-f1}, \ref{fig:CR-distr-real-l0-f2},  and \ref{fig:CR-distr-real-l0-f3}. GAN with linear activation (epoch 1250): \ref{fig:CR-distr-LA-l0-f0}, \ref{fig:CR-distr-LA-l0-f1}, \ref{fig:CR-distr-LA-l0-f2} and \ref{fig:CR-distr-LA-l0-f3}. GAN with custom activation (epoch 850): \ref{fig:CR-distr-LS-l0-f0}, \ref{fig:CR-distr-LS-l0-f1}, \ref{fig:CR-distr-LS-l0-f2} and\ref{fig:CR-distr-LS-l0-f3}.}
\label{fig:CR-distr-l0}
\end{figure*}



%%%%%%%%%
% et1
%%%%%%%%%


\begin{figure*}[!t]
\centering

\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F0_CR_et1_REAL.png} 
\caption{Feat 0. Real data.}\label{fig:CR-distr-real-l1-f0}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F0_CR_et1_FA_l.png} 
\caption{Feat 0. Linear activation.}\label{fig:CR-distr-LA-l1-f0}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F0_CR_et1_FA_S.png} 
\caption{Feat 0. Custom activation.}\label{fig:CR-distr-LS-l1-f0}
\end{subfigure}

\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F1_CR_et1_REAL.png} 
\caption{Feat 1. Real data.}\label{fig:CR-distr-real-l1-f1}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F1_CR_et1_FA_l.png} 
\caption{Feat 1. Linear activation.}\label{fig:CR-distr-LA-l1-f1}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F1_CR_et1_FA_S.png} 
\caption{Feat 1. Custom activation.}\label{fig:CR-distr-LS-l1-f1}
\end{subfigure}

\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F2_CR_et1_REAL.png} 
\caption{Feat 2. Real data.}\label{fig:CR-distr-real-l1-f2}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F2_CR_et1_FA_l.png} 
\caption{Feat 2. Linear activation.}\label{fig:CR-distr-LA-l1-f2}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F2_CR_et1_FA_S.png} 
\caption{Feat 2. Custom activation.}\label{fig:CR-distr-LS-l1-f2}
\end{subfigure}

\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F3_CR_et1_REAL.png} 
\caption{Feat 3. Real data.}\label{fig:CR-distr-real-l1-f3}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F3_CR_et1_FA_l.png} 
\caption{Feat 3. Linear activation.}\label{fig:CR-distr-LA-l1-f3}
\end{subfigure}
\begin{subfigure}[t]{.32\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/H_F3_CR_et1_FA_S.png} 
\caption{Feat 3. Custom activation.}\label{fig:CR-distr-LS-l1-f3}
\end{subfigure}

\caption{Cryptomining data set. Frequency distribution histogram of the 4 variables extracted from cryptomining traffic (Label 1). Real data distribution: \ref{fig:CR-distr-real-l1-f0}, \ref{fig:CR-distr-real-l1-f1}, \ref{fig:CR-distr-real-l1-f2},  and \ref{fig:CR-distr-real-l1-f3}. GAN with linear activation (epoch 1250): \ref{fig:CR-distr-LA-l1-f0}, \ref{fig:CR-distr-LA-l1-f1}, \ref{fig:CR-distr-LA-l1-f2} and \ref{fig:CR-distr-LA-l1-f3}. GAN with custom activation (epoch 850): \ref{fig:CR-distr-LS-l1-f0}, \ref{fig:CR-distr-LS-l1-f1}, \ref{fig:CR-distr-LS-l1-f2} and\ref{fig:CR-distr-LS-l1-f3}.}
\label{fig:CR-distr-l1}
\end{figure*}

==> figuras/fig-FA-LR.tex <==
\begin{figure*}[!hp]
\begin{mdframed}
\centering

\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/FA-LR_1rnd_0-1_400-4_Testing.png} 
  \includegraphics[width=0.49\linewidth]{images/FA-LR_1rnd_0-1_400-4_Training.png}}
\caption{Policy \ref{enum:poli-vainilla-1}). Training with 400K/4K distribution and one generator chosen uniformly at random}\label{fig:FA_400K-4K}
\end{subfigure}
%


\medskip

\begin{subfigure}[t]{.99\textwidth}
\centering
\vspace{0pt}% set the real top as the top
\includegraphics[width=0.49\linewidth]{images/FA-LR_2rnd_0-1_400-4_Testing.png}
\hfill
\includegraphics[width=0.49\linewidth]{images/FA-LR_2rnd_0-1_400-4_Training.png}
\caption{Policy \ref{enum:poli-vainilla-2}). Training with 400K/4K distribution and a mix of two generators is chosen uniformly at random}\label{fig:FA-2_400K-4K}
\end{subfigure}
%

\medskip
\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/FA-LR_1rnd_0-1_4-4_Testing.png} 
  \includegraphics[width=0.49\linewidth]{images/FA-LR_1rnd_0-1_4-4_Training.png}}
\caption{Policy \ref{enum:poli-vainilla-4}). Training with 4K/4K distribution and one generator chosen uniformly at random}\label{fig:FA_4K-4K}
\end{subfigure}
%
\end{mdframed}
\medskip
\begin{minipage}[t]{.99\textwidth}
\caption{$F_1$-score on testing (left) and training (right) using a generator with custom activation functions at the output and policies \ref{enum:poli-vainilla-1}), \ref{enum:poli-vainilla-2}) and \ref{enum:poli-vainilla-4}) (subsection \ref{sec:custom-act-func}). Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented.} \label{fig:FA}
\end{minipage}

\end{figure*}

==> figuras/fig-Mean.tex <==

\begin{figure*}[!tb]
\begin{mdframed}
\centering

\begin{subfigure}[t]{0.99\textwidth}
\centering
\includegraphics[width=0.49\linewidth]{images/Mean_0-1_400-4_Testing.png} \includegraphics[width=0.49\linewidth]{images/Mean_0-1_400-4_Training.png}
\caption{Unbalanced dataset with the original 400K/4K distribution.}\label{fig:mean_400K-4K}
\end{subfigure}
%

\medskip

\begin{subfigure}[t]{.99\textwidth}
\centering
\vspace{0pt}% set the real top as the top
\includegraphics[width=0.49\linewidth]{images/Mean_0-1_4-4_Testing.png} \includegraphics[width=0.49\linewidth]{images/Mean_0-1_4-4_Training.png}
\caption{Balanced dataset with 4K/4K distribution.}\label{fig:mean_4K-4K}
\end{subfigure}
%
%
\end{mdframed}

\medskip
%\vspace{1ex}
\begin{minipage}[b]{.99\textwidth}
\caption{$F_1$-score on testing (left) and training (right) using a na\"ive mean-based generator with unbalanced and balanced datasets for training (subsection \ref{sec:naive-exp}). Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented. 
%In (\subref{fig:real_400K-4K}) 400K/4K data distribution was used in tragreen square....
} \label{fig:mean}
\end{minipage}

\end{figure*}



==> figuras/fig-Real.tex <==

\begin{figure*}[!h]
\begin{mdframed}
\centering

\begin{subfigure}[t]{0.99\textwidth}
\includegraphics[width=0.49\linewidth]{images/Real_0-1_400-4_Testing.png} 
\includegraphics[width=0.49\linewidth]{images/Real_0-1_400-4_Training.png}
\caption{F1-score on testing (left) and training (right) using real data for training and testing (400K/4K distribution).}\label{fig:real_400K-4K}
\end{subfigure}
%


\medskip

\begin{subfigure}[t]{.99\textwidth}
\centering
\vspace{0pt}% set the real top as the top
\includegraphics[width=0.49\linewidth]{images/Real_0-1_4-4_Testing.png} \includegraphics[width=0.49\linewidth]{images/Real_0-1_4-4_Training.png}
\caption{F1-score on testing (left) and training (right) using real data for training and testing (4K/4K distribution).}\label{fig:real_4K-4K}
\end{subfigure}
%


%
\end{mdframed}
\medskip
\begin{minipage}[t]{.99\textwidth}
\caption{$F_1$-score on testing (left) and training (right) using real data  with 400K/4K (\subref{fig:real_400K-4K}) and 4K/4K (\subref{fig:real_4K-4K}) class distributions for training (subsection \ref{sec:experiments-real}). Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented.} \label{fig:real}
\end{minipage}
\end{figure*}


==> figuras/fig-Vainilla-DKJ.tex <==
\begin{figure*}[!h]
\begin{mdframed}
\centering

\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/Vainilla_DK_top10_1rnd_0-1_4-4_Testing.png} 
  \includegraphics[width=0.49\linewidth]{images/Vainilla_DK_top10_1rnd_0-1_4-4_Training.png}}
\caption{Using top $10$ models sorted by $L^1$ distance}
\end{subfigure}
%
\medskip

\begin{subfigure}[t]{.99\textwidth}
\centering
\vspace{0pt}% set the real top as the top
\includegraphics[width=0.49\linewidth]{images/Vainilla_DJ_top10_1rnd_0-1_4-4_Testing.png}
\hfill
\includegraphics[width=0.49\linewidth]{images/Vainilla_top10_Pos_1rnd_0-1_400-4_Training.png}
\caption{Using top $10$ models sorted by Jaccard index} 
\end{subfigure}

%
\end{mdframed}
\medskip
\begin{minipage}[t]{.99\textwidth}
\caption{
$F1-score$ on testing (left) and training (right) with sampling elitism using policy \ref{enum:poli-vainilla-1}). Elitism of the top $10$ sorted by statistical coefficients (subsection \ref{sec:elit-metrics}. Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented.} \label{fig:vainilla-top10-DKJ}
\end{minipage}

\end{figure*}

==> figuras/fig-Vainilla-Pos.tex <==
\begin{figure*}[!htp]
\begin{mdframed}
\begin{subfigure}[t]{1.\textwidth}
\centerline{
    \includegraphics[width=0.49\linewidth]{images/Vainilla_1rnd_positivos_0-1_400-4_Testing.png} 
    \includegraphics[width=0.49\linewidth]{images/Vainilla_1rnd_positivos_0-1_400-4_Training.png}}

\end{subfigure}

\begin{minipage}[t]{1.\textwidth}
\caption{$F1-score$ on testing (left) and training (right) using the discriminator as a quality assurance filter (subsection  \ref{sec:discr-quality-assurance}). Training with 400K/4K distribution. Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented.}
\label{fig:vainillaPos_400K-4K}
\end{minipage}
\end{mdframed}
\end{figure*}



==> figuras/fig-Vainilla-top10.tex <==
\begin{figure*}[!h]
\begin{mdframed}
\centering

\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/Vainilla_top10_1rnd_0-1_400-4_Testing.png} 
  \includegraphics[width=0.49\linewidth]{images/Vainilla_top10_1rnd_0-1_400-4_Training.png}}
\caption{Training with 400K/4K distribution. 1 generator chosen uniformly at random}\label{fig:vainilla-top10_400K-4K}
\end{subfigure}
%
\medskip

\begin{subfigure}[t]{.99\textwidth}
\centering
\vspace{0pt}% set the real top as the top
\includegraphics[width=0.49\linewidth]{images/Vainilla_top10_Pos_1rnd_0-1_400-4_Testing.png}
\hfill
\includegraphics[width=0.49\linewidth]{images/Vainilla_top10_Pos_1rnd_0-1_400-4_Training.png}
\caption{Training with 400K/4K distribution. 1 generator chosen uniformly at random} filtering positive values\label{fig:vainilla-Pos-top10_400K-4K}
\end{subfigure}

\medskip
\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/Vainilla_top10_1rnd_0-1_4-4_Testing.png} 
  \includegraphics[width=0.49\linewidth]{images/Vainilla_top10_1rnd_0-1_4-4_Training.png}}
\caption{Training with 4K/4K distribution. 1 generator chosen uniformly at random}\label{fig:vainilla-top10_4K-4K}
\end{subfigure}
%
\end{mdframed}
\medskip
\begin{minipage}[t]{.99\textwidth}
\caption{$F_1$-score on testing (left) and training (right) with sampling elitism among the top $10$ models in training sorted by $F_1$-score (subsection \ref{subsec:elit_f1}). Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented.} \label{fig:vainilla-top10}
\end{minipage}

\end{figure*}

==> figuras/fig-Vainilla.tex <==
\begin{figure*}[!hp]
\begin{mdframed}
\centering

\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/Vainilla_1rnd_0-1_400-4_Testing.png} 
  \includegraphics[width=0.49\linewidth]{images/Vainilla_1rnd_0-1_400-4_Training.png}}
\caption{Policy \ref{enum:poli-vainilla-1}). Training with 400K/4K distribution and one generator chosen uniformly at random}\label{fig:vainilla_400K-4K}
\end{subfigure}
%
\medskip

\begin{subfigure}[t]{.99\textwidth}
\centering
\vspace{0pt}% set the real top as the top
\includegraphics[width=0.49\linewidth]{images/Vainilla_2rnd_0-1_400-4_Testing.png}
\hfill
\includegraphics[width=0.49\linewidth]{images/Vainilla_2rnd_0-1_400-4_Training.png}
\caption{Policy \ref{enum:poli-vainilla-2}). Training with 400K/4K distribution and a mix of two generators is chosen uniformly at random}\label{fig:vainilla2_400K-4K}
\end{subfigure}

\medskip
\begin{subfigure}[t]{0.99\textwidth}
\centerline{
  \includegraphics[width=0.49\linewidth]{images/Vainilla_1rnd_0-1_4-4_Testing.png} 
  \includegraphics[width=0.49\linewidth]{images/Vainilla_1rnd_0-1_4-4_Training.png}}
\caption{Policy \ref{enum:poli-vainilla-4}). Training with 4K/4K distribution and one generator chosen uniformly at random}\label{fig:vainilla_4K-4K}
\end{subfigure}
%
\end{mdframed}
\medskip
\begin{minipage}[t]{.99\textwidth}
\caption{$F_1$-score on testing (left) and training (right) using a standard GAN generator and sampling policies \ref{enum:poli-vainilla-1}), \ref{enum:poli-vainilla-2}) and \ref{enum:poli-vainilla-4}) (subsection \ref{sec:results-standard-GAN}). Results for decision thresholds of 0.2, 0.4, 0.5, 0.6 and 0.8 are represented.} \label{fig:vainilla}
\end{minipage}

\end{figure*}

==> figuras/fig_distancias_et0.tex <==


%%%%%%%%%
% et0
%%%%%%%%%


\begin{figure*}[!t]

\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et0_f1_test.png} 
\caption{$F_1$-score on testing}
\label{fig:vainilla-f1}
\end{subfigure}
%
\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et0_kolmo.png} 
\caption{$L^1$ distance}
\label{fig:vainilla-kolmo}
\end{subfigure}

\medskip

\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et0_jacc.png} 
\caption{Jaccard index}
\label{fig:vainilla-jac}
\end{subfigure}
%
\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et0_jacc99.png} 
\caption{Jaccard index from percentile 1}
\label{fig:vainilla-jac-1}
\end{subfigure}


\caption{Evolution of $F_1$-score on testing, $L^1$ distance and Jaccard index using GAN generator for label 0. The $x$-axis represents the GAN training epochs.}
\label{fig:distances-vainilla}
\end{figure*}


==> figuras/fig_distancias_et1.tex <==

%%%%%%%%%
% et1
%%%%%%%%%



\begin{figure*}[!t]


\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[trim=0.5cm 0.1cm 2.8cm 0.1cm, clip=true, width=1\linewidth]{images/et1_f1_test.png} 
\caption{$F_1$-score on testing}\label{fig:vainilla-f1-et1}
\end{subfigure}
%
\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et1_kolmo.png} 
\caption{$L^1$ distance}\label{fig:vainilla-kolmo-et1}
\end{subfigure}

\medskip

\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et1_jacc.png} 
\caption{Jaccard index}\label{fig:vainilla-jacc-et1}
\end{subfigure}
%
\begin{subfigure}[t]{.48\textwidth}
\centering
\includegraphics[width=1\linewidth]{images/et1_jacc99.png} 
\caption{Jaccard index from percentile 1}\label{fig:vainilla-jacc-1-et1}
\end{subfigure}


\caption{Evolution of $F_1$-score on testing, $L^1$ distance and Jaccard index using GAN generator for label 1. The $x$-axis represents GAN training epochs.}
\label{fig:distances-vainilla-et1}
\end{figure*}

==> figuras/fig_distr_et0-et1.tex <==


%%%%%%%%%
% et0
%%%%%%%%%



\begin{figure*}[!t]
\centering
%et0
\centering
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_distr_1.png} 
\caption{Label 0. Epoch 1}\label{fig:distr-l0-1}
\end{subfigure}
%
%hspace*{\fill}
%\hspace*{3em}
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_distr_5.png} 
\caption{Label 0. Epoch 5}\label{fig:distr-l0-5}
\end{subfigure}
%
%\medskip
%
%\centering
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_distr_200.png} 
\caption{Label 0. Epoch 200}\label{fig:distr-l0-200}
\end{subfigure}
%
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_distr_800.png} 
\caption{Label 0. Epoch 800}\label{fig:distr-l0-800}
\end{subfigure}
%\hspace*{3em}
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_distr_1500.png} 
\caption{Label 0. Epoch 1000}\label{fig:distr-l0-1500}
\end{subfigure}

\medskip

%et1
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_distr_1.png} 
\caption{Label 1. Epoch 1}\label{fig:distr-l1-1}
\end{subfigure}
%
%hspace*{\fill}
%\hspace*{3em}
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_distr_5.png} 
\caption{Label 1. Epoch 5}\label{fig:distr-l1-5}
\end{subfigure}
%
%\medskip
%
%\centering
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_distr_200.png} 
\caption{Label 1. Epoch 200}\label{fig:distr-l1-200}
\end{subfigure}
%
%\hspace*{3em}
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_distr_800.png} 
\caption{Label 1. Epoch 800}\label{fig:distr-l1-800}
\end{subfigure}
%
\begin{subfigure}[t]{.195\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_distr_1500.png} 
\caption{Label 1. Epoch 1500}\label{fig:distr-l1-1500}
\end{subfigure}
\caption{Comparison of synthetic (blue) and real (red) data distributions using GAN generators for label 0 (\ref{fig:distr-l0-1}, \ref{fig:distr-l0-5}, \ref{fig:distr-l0-200}, \ref{fig:distr-l0-800} and \ref{fig:distr-l0-1500}) and label 1 (\ref{fig:distr-l1-1}, \ref{fig:distr-l1-5}, \ref{fig:distr-l1-200}, \ref{fig:distr-l1-800} and \ref{fig:distr-l1-1500}) in different epochs (1, 5, 200, 800 and 1500). The $4$-dimensional vector has been flattened into by sorting by frequency in ascending order on the $x$-axis.}
\label{fig:comparison-vainilla}
\end{figure*}

==> figuras/fig_real_distr_et0_et1.tex <==

%%%%%%%%%
% et0
%%%%%%%%%



\begin{figure*}[!t]
\centering
%et0
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_f0_real.png} 
\caption{Label 0. Feature 1}\label{fig:distr-real-l0-f1}
\end{subfigure}
%
%hspace*{\fill}
%\hspace*{3em}
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_f1_real.png} 
\caption{Label 0. Feature 2}\label{fig:distr-real-l0-21}
\end{subfigure}
%
%\medskip
%
%\centering
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_f2_real.png} 
\caption{Label 0. Feature 3}\label{fig:distr-real-l0-f3}
\end{subfigure}
%
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et0_f3_real.png} 
\caption{Label 0. Feature 4}\label{fig:distr-real-l0-f4}
\end{subfigure}
%\hspace*{3em}


\medskip

%et0
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_f0_real.png} 
\caption{Label 1. Feature 1}\label{fig:distr-real-l1-f1}
\end{subfigure}
%
%hspace*{\fill}
%\hspace*{3em}
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_f1_real.png} 
\caption{Label 1. Feature 2}\label{fig:distr-real-l1-f2}
\end{subfigure}
%
%\medskip
%
%\centering
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_f2_real.png} 
\caption{Label 1. Feature 3}\label{fig:distr-real-l1-f3}
\end{subfigure}
%
\begin{subfigure}[t]{.245\textwidth}
%\centering
\includegraphics[width=1\linewidth]{images/et1_f3_real.png} 
\caption{Label 1. Feature 4}\label{fig:distr-real-l1-f4}
\end{subfigure}
%\hspace*{3em}


\caption{Frequency distribution histogram of the 4 variables extracted from normal (Label 0) and cryptomining (label 1) traffic. Label 0 (\ref{fig:distr-l0-1}, \ref{fig:distr-l0-5}, \ref{fig:distr-l0-200}, \ref{fig:distr-l0-800} and \ref{fig:distr-l0-1500}) and label 1 (\ref{fig:distr-l1-1}, \ref{fig:distr-l1-5}, \ref{fig:distr-l1-200}, \ref{fig:distr-l1-800} and \ref{fig:distr-l1-1500}) }
\label{fig:real-data-distribution}
\end{figure*}

==> tablas/hyperparameters.tex <==
% \usepackage{array}
% \usepackage{graphicx}


\begin{table*}[!t]
\centering
\caption{GAN hyperparameters.}
\label{table:hyperparameters}
\resizebox{0.67\linewidth}{!}{%
\begin{tabular}{>{\hspace{0pt}}m{0.0027\linewidth}>{\hspace{0pt}}m{0.184\linewidth}|>{\hspace{0pt}}m{0.272\linewidth}|>{\hspace{0pt}}m{0.184\linewidth}|}
 & \multicolumn{1}{>{\hspace{0pt}}m{0.204\linewidth}}{} &  & \textbf{Range of values} \\ 
\cline{2-4}
 & \textbf{Generator/discriminator}\par{}\textbf{FCNN architectures} & \textit{\# layers} & {[}2..6] \\ 
\cline{2-4}
 &  & \textit{\# units per layer} & {[}100..10000] \\ 
\cline{2-4}
 & \textbf{Generator} & \textit{Output Activation~} & (linear,custom) \\ 
\cline{2-4}
 &  & Output filtering with discriminator \par{}(\textgreater{}0, percentile) & (True,False)\par{}{[}0..100] \\ 
\cline{3-4}
 &  & \textit{Latent vector }\par{}\textit{with Embedding (categories)} & (True,False)\par{}{[}1..20] \\ 
\cline{3-4}
 &  & latent vector & Fixed 123 \\ 
\cline{3-4}
 &  & noise for latent vector (distr,std) & (normal, uniform)\par{}std=[0.1..100] \\ 
\cline{3-4}
 &  & batch normalization & {[}True..False] \\ 
\cline{3-4}
 &  & regularization: L2, dropout & Fixed values (0,0) \\ 
\cline{3-4}
 &  & learning rate & Default value (0.001) \\ 
\cline{3-4}
 &  & LeakyRelu alpha & Fixed value (0.15) \\ 
\cline{3-4}
 &  & \textit{Percentage of tanh/LeakyRelu }\par{}\textit{in internal units} & {[}0..100] \\ 
\cline{2-4}
 & \textbf{Discriminator}\par{} & \textit{Noise in fakes }\par{}\textit{(distribution,std)} & (normal,uniform)\par{}{[}0..20] \\ 
\cline{2-4}
 &  & \textit{Noise in all examples}\par{}\textit{(distribution,std)} & (normal,uniform)\par{}{[}0..20] \\ 
\cline{3-4}
 &  & \textit{Ratio Label change} & {[}0..20] \\ 
\cline{3-4}
 &  & batch normalization & {[}True..False] \\ 
\cline{3-4}
 &  & regularization: L2, dropout & {[}0..2], [0..30] \\ 
\cline{3-4}
 &  & LeakyRelu alpha & Fixed value (0.2) \\ 
\cline{3-4}
 &  & learning rate & {[}0.0001..0.001] \\ 
\cline{2-4}
 & \textbf{Adaptive~mini-batch} & \textit{generator. ratio fake pass} & Fixed (0.3) \\ 
\cline{2-4}
 &  & \textit{discriminator. ratio TP} & Fixed (0.01) \\ 
\cline{3-4}
 &  & \textit{discriminator. ratio TN} & Fixed (0.01) \\
\cline{3-4}
\end{tabular}
}
\end{table*}

==> tablas/tabla1.tex <==

%\begin{table}
%\centering
%\caption{Tabla Pepito}
\resizebox{\linewidth}{!}{%
\begin{tabular}{>{\hspace{0pt}}m{0.175\linewidth}|>{\hspace{0pt}}m{0.215\linewidth}|>{\hspace{0pt}}m{0.261\linewidth}|>{\hspace{0pt}}m{0.261\linewidth}|}
\multicolumn{1}{>{\hspace{0pt}}m{0.175\linewidth}}{} &                                                            & Best                                 & Default                               \\ 
\hline
\textbf{400K/4K }\par{}\textbf{1 model}              & \textit{\textbf{threshold}}                                & ~0.8                                 & 0.5                                   \\ 
\hline
                                                     & \textit{\textbf{F1-score}}                                 & 0.927                                & 0.915                                 \\ 
\cline{2-4}
                                                     & \textbf{\textit{Confusion }}\par{}\textbf{\textit{matrix}} & {[}399449 551] \par{}[ 701 ~~~~3687] & {[}399601 399] \par{}[ 983 ~~~~3405]  \\
\cline{2-4}
\end{tabular}
}
%\end{table}

==> tablas/tabla_Baseline_Medias.tex <==
% \usepackage{array}
% \usepackage{graphicx}

\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Baseline results using a naive mean-based generator for training. }
\label{table:mean}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Mean-based generation}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.732 & 0.664 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 396318 & 3682 \\\hline 1894 & 2493 \end{tabular} & \begin{tabular}{c|c} 390060 & 9940 \\\hline 1416 & 2971 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Mean-based generation}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.601 & 0.583 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 377352 & 22648 \\\hline 839 & 3548 \end{tabular} & \begin{tabular}{c|c} 370528 & 29472 \\\hline 537 & 3850 \end{tabular}\\ \hline
\end{tabular}
}
}

\end{table*}


==> tablas/tabla_FA-Leaky.tex <==
\begin{table}[h!]
%
\parbox{.48\linewidth}{
\caption{Generators using a custom activation function in the output. Results in testing using the best models in training.}
\label{table:FA-Leaky}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-1}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.649 & 0.555 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 382755 & 17245 \\\hline  241 & 4146 \end{tabular} & \begin{tabular}{c|c} 357385 & 42615 \\\hline 96 & 4291\end{tabular}\\ \hline\hline
 
 
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-2}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.622 & 0.559 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 377693 & 22307] \\\hline 163 & 4224\end{tabular} & \begin{tabular}{c|c} 358897 & 41103 \\\hline 82 & 4305 \end{tabular}\\ \hline\hline
 
 
 
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-4}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.532 & 0.467 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 345452 & 54548] \\\hline 21 & 4366\end{tabular} & \begin{tabular}{c|c} 298568 & 101432] \\\hline 0 & 4387\end{tabular}\\ \hline
\end{tabular}
}
}
\end{table}

==> tablas/tabla_FA-linear-top10.tex <==
\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Results in testing by sampling with elitism among the top $10$ models in training sorted by $F_1$-score. Linear activation function were used in the output layer.}
\label{tab:FA-linear-top10}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top $10$ in $F_1$-score}\end{matrix}$}  & \textit{{Threshold}} & 0.4 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} &  0.951 & 0.950 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399800 & 200 \\\hline 608 & 3780 \end{tabular} & \begin{tabular}{c|c} 399832 & 168 \\\hline 658& 3730 \end{tabular}\\ \hline
\end{tabular}
}
}
\end{table*}

==> tablas/tabla_FA-linear.tex <==
\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Performance metrics of in testing using the best models in training with a synthetic dataset generated by a standard GAN.}
\label{tab:vainilla}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-1}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.4 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.936 & 0.933 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399926 & 74 \\\hline 927 & 3461 \end{tabular} & \begin{tabular}{c|c} 399962 & 38 \\\hline 998 & 3390 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-2}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.927  & 0.915 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399449 & 551 \\\hline 701 & 3687\end{tabular} & \begin{tabular}{c|c} 399601 & 399] \\\hline 983 & 3405 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-4}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.878 & 0.835 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399030 & 970 \\\hline 1108 & 3280\end{tabular} & \begin{tabular}{c|c} 396381 & 3619 \\\hline 315 & 4073 \end{tabular}\\ \hline
\end{tabular}
}
}
\end{table*}


==> tablas/tabla_FA-lnear-top10-KJ-dist.tex <==
\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Generators using linear activation function in the output. Results in testing using the best among the top 10 models in training with $L^1$-distance and Jaccard index.}
\label{tab:FA-linear-top10-dKJ}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top 10 $L^1$-distance}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.869 & 0.858 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399491 & 509 \\\hline 1506 & 2882 \end{tabular} & \begin{tabular}{c|c} 398536 & 1464 \\\hline 1094 & 3294 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top 10 Jaccard index}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.884  & 0.826 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399033 & 967 \\\hline 1031 & 3357\end{tabular} & \begin{tabular}{c|c} 396881 & 3119 \\\hline 720 & 3668 \end{tabular}\\ \hline
\end{tabular}
}
}
\end{table*}

==> tablas/tabla_FA-top10.tex <==



\begin{table*}[tp]
%
\parbox{.48\linewidth}{
\caption{Generators using linear activation function in the output. Results in testing using the best among top 10 models in training with F1-score }
\label{tab:FA-linear-top10}
\centering
\resizebox{.99\linewidth}{!}{%
\input{tablas/tabla_FA-linear-top10}
}
}
\hfill
\parbox{.48\linewidth}{
\caption{Generators using linear activation function in the output. Results in testing using the best among the top 10 models in training with Kolmogorov distance and Jaccard index}
\label{tab:FA-linear-top10-dKJ}
\centering
\resizebox{.99\linewidth}{!}{%
\input{tablas/tabla_FA-lnear-top10-KJ-dist}
}
}
\end{table*}%



==> tablas/tabla_FA_filtering.tex <==
\begin{table*}[h!]
%
\parbox{.48\linewidth}{
\caption{Performance metrics of in testing using the best models in training after filtering fake samples.}
\label{tab:filtering}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Filtering out fakes}\end{matrix}$}  & \textit{{Threshold}} & 0.6 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.925 & 0.914 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399511 & 489 \\\hline 767 & 3621 \end{tabular} & \begin{tabular}{c|c} 399221 & 779 \\\hline 722 & 3666 \end{tabular}\\ \hline\hline
\end{tabular}
}
}
\end{table*}


==> tablas/tabla_baseline.tex <==
\begin{table*}[t!]
%
\parbox{.48\linewidth}{
\caption{Baseline results using real data for training.}
\label{table:real}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Real dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.4 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.962 & 0.928 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399817 & 183 \\\hline 459 & 3929 \end{tabular} & \begin{tabular}{c|c} 399877 & 123 \\\hline 1008 & 3380 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Real dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.919 & 0.793 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 398602 & 1398 \\\hline 197 & 4191 \end{tabular} & \begin{tabular}{c|c} 394172 & 5828 \\\hline 62 & 4326 \end{tabular}\\ \hline
\end{tabular}
}
}
\hfill
\parbox{.48\linewidth}{
\caption{Baseline results using a naive mean-based generator for training. }
\label{table:mean}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Mean-based generation}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.732 & 0.664 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 396318 & 3682 \\\hline 1894 & 2493 \end{tabular} & \begin{tabular}{c|c} 390060 & 9940 \\\hline 1416 & 2971 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Mean-based generation}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.601 & 0.583 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 377352 & 22648 \\\hline 839 & 3548 \end{tabular} & \begin{tabular}{c|c} 370528 & 29472 \\\hline 537 & 3850 \end{tabular}\\ \hline
\end{tabular}
}
}
\medskip
\vspace{3ex}

\parbox{.48\linewidth}{
\caption{Performance of synthetic traffic generated by standard WGANs. Results on testing using the best models on training.}
\label{tab:vainilla}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-1}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.4 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.936 & 0.933 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399926 & 74 \\\hline 927 & 3461 \end{tabular} & \begin{tabular}{c|c} 399962 & 38 \\\hline 998 & 3390 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-2}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.927  & 0.915 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399449 & 551 \\\hline 701 & 3687\end{tabular} & \begin{tabular}{c|c} 399601 & 399 \\\hline 983 & 3405 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-4}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.878 & 0.835 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399030 & 970 \\\hline 1108 & 3280\end{tabular} & \begin{tabular}{c|c} 396381 & 3619 \\\hline 315 & 4073 \end{tabular}\\ \hline
\end{tabular}
}
}
\hfill
\parbox{.48\linewidth}{
\caption{Performance of synthetic traffic when generators use  custom activation functions in the output. Results on testing using the best models on training.}
\label{table:FA-Leaky}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-1}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.649 & 0.555 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 382755 & 17245 \\\hline  241 & 4146 \end{tabular} & \begin{tabular}{c|c} 357385 & 42615 \\\hline 96 & 4291\end{tabular}\\ \hline\hline
 
 
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-2}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.622 & 0.559 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 377693 & 22307 \\\hline 163 & 4224\end{tabular} & \begin{tabular}{c|c} 358897 & 41103 \\\hline 82 & 4305 \end{tabular}\\ \hline\hline
 
 
 
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 4K/4K }\\\textbf{Policy \ref{enum:poli-vainilla-4}) dataset}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.532 & 0.467 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 345452 & 54548] \\\hline 21 & 4366\end{tabular} & \begin{tabular}{c|c} 298568 & 101432 \\\hline 0 & 4387\end{tabular}\\ \hline
\end{tabular}
}
}

\medskip
\vspace{3ex}
\parbox{.48\linewidth}{
\caption{Performance of synthetic traffic generated by standard WGANs after filtering fake samples by discriminator. Results on testing using the best models on training.}
\label{tab:filtering}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Filtering out fakes}\end{matrix}$}  & \textit{{Threshold}} & 0.6 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.925 & 0.914 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399511 & 489 \\\hline 767 & 3621 \end{tabular} & \begin{tabular}{c|c} 399221 & 779 \\\hline 722 & 3666 \end{tabular}\\ \hline\hline
\end{tabular}
}
%
\vspace{3ex}
\caption{Performance of synthetic traffic generated by standard WGANs by sampling generators with elitism among the top $10$ models in training sorted by $F_1$-score. Results on testing.}
\label{tab:FA-linear-top10}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top $10$ in $F_1$-score}\end{matrix}$}  & \textit{{Threshold}} & 0.4 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} &  0.951 & 0.950 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399800 & 200 \\\hline 608 & 3780 \end{tabular} & \begin{tabular}{c|c} 399832 & 168 \\\hline 658& 3730 \end{tabular}\\ \hline
\end{tabular}
}
}
%
\hfill
\parbox{.48\linewidth}{
\caption{
Performance of synthetic traffic generated by standard WGANs by sampling generators with elitism among the top $10$ models in training sorted by $L^1$-distance and Jaccard index. Results on testing.}
\label{tab:FA-linear-top10-dKJ}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline \textbf{Dataset} & \textbf{Quality Measure} & \textbf{Best} & \textbf{Default} \\\hline\hline
\multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top 10 $L^1$-distance}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5  \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.869 & 0.858 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399491 & 509 \\\hline 1506 & 2882 \end{tabular} & \begin{tabular}{c|c} 398536 & 1464 \\\hline 1094 & 3294 \end{tabular}\\ \hline\hline
 
 \multirow{3}{*}{\vspace{-0.3cm}$\begin{matrix}\textbf{Training 400K/4K }\\\textbf{Top 10 Jaccard index}\end{matrix}$}  & \textit{{Threshold}} & 0.8 & 0.5 \\ 
\cline{2-4} & \textit{{$F_1$-score}} & 0.884  & 0.826 \\ \cline{2-4}
 & $\begin{matrix}\textit{{Confusion }} \\ \textit{{matrix}}\end{matrix}$ & \begin{tabular}{c|c} 399033 & 967 \\\hline 1031 & 3357\end{tabular} & \begin{tabular}{c|c} 396881 & 3119 \\\hline 720 & 3668 \end{tabular}\\ \hline
\end{tabular}
}
}

\end{table*}

